Cross-Media Keyphrase Prediction: A Unified Framework with Multi-Modality Multi-Head Attention and Image Wordings

Social media produces large amounts of contents every day. To help users quickly capture what they need, keyphrase prediction is receiving a growing attention. Nevertheless, most prior efforts focus on text modeling, largely ignoring the rich features embedded in the matching images. In this work, we explore the joint effects of texts and images in predicting the keyphrases for a multimedia post. To better align social media style texts and images, we propose: (1) a novel Multi-Modality Multi-Head Attention (M3H-Att) to capture the intricate cross-media interactions; (2) image wordings, in forms of optical characters and image attributes, to bridge the two modalities. Moreover, we design a unified framework to leverage the outputs of keyphrase classification and generation and couple their advantages. Extensive experiments on a large-scale dataset newly collected from Twitter show that our model significantly outperforms the previous state of the art based on traditional attention networks. Further analyses show that our multi-head attention is able to attend information from various aspects and boost classification or generation in diverse scenarios.

==> tables/more_m3h_att_vis.tex <==
\begin{table}
\begin{center}
\resizebox{0.5\textwidth}{!}{

\begin{tabular}{p{4.8cm}p{4.8cm}p{4.8cm}}
 \begin{minipage}{\textwidth}
      \includegraphics[width=4.8cm,height=4.8cm]{figures/book_12_2.pdf}
\end{minipage}
 & 
 \begin{minipage}{\textwidth}
      \includegraphics[width=4.8cm,height=4.8cm]{figures/book_12_6.pdf}
\end{minipage}
 & 
 \begin{minipage}{\textwidth}
      \includegraphics[width=4.8cm,height=4.8cm]{figures/book_12_7.pdf}
\end{minipage}
 \\
 \multicolumn{1}{c}{\huge{Head 0}} &
  \multicolumn{1}{c}{\huge{Head 5}} &
   \multicolumn{1}{c}{\huge{Head 9}}
\\
 \begin{minipage}{\textwidth}
      \includegraphics[width=4.8cm,height=4.8cm]{figures/dog_12_6.pdf}
\end{minipage}
 & 
 \begin{minipage}{\textwidth}
      \includegraphics[width=4.8cm,height=4.8cm]{figures/dog_12_9.pdf}
\end{minipage}
 & 
 \begin{minipage}{\textwidth}
      \includegraphics[width=4.8cm,height=4.8cm]{figures/dog_12_10.pdf}
\end{minipage}
 \\
 \multicolumn{1}{c}{\huge{Head 0}} &
  \multicolumn{1}{c}{\huge{Head 5}} &
   \multicolumn{1}{c}{\huge{Head 9}}
\end{tabular}

}
\end{center}
\vspace{-0.5em}
\captionsetup{type=figure}
\caption{Attention weight visualization for some selected heads on the grid-level VGG image features.
}\label{tables:more_m3h_att_vis}
\vspace{-0.5em}
\end{table}


==> tables/text_image_relationship.tex <==
\begin{table}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccc}
\toprule
 & Image adds & Image does not add\\
\midrule
% F1@1 scores
Text is
 & \multirow{2}{*}{53.90/48.13~(48\%)} & \multirow{2}{*}{50.45/39.90~(25\%)} \\
represented & & \\

\midrule

Text is not
 & \multirow{2}{*}{44.94/34.92~(15\%)} & \multirow{2}{*}{34.90/26.52~(12\%)} \\
represented & & \\

\bottomrule
\end{tabular}
}

%  \vskip -0.5em

\caption{Comparison F1@1 scores between our model and \textsc{seq2seq-copy} (separated by ``/'') on 
% a sampled subset data, broken down by 
four different types of text-image relationship. The $\%$ values in the parentheses denote the data proportion. ``Text is represented'' takes up a larger percentage as we filter out tweets with fewer than $5$ tokens during preprocessing.
}\label{tabs:relationship}
\vspace{-0.5em}

\end{table}

